ReFiNe: Recursive Field Networks for Cross-modal Multi-scene Representation

The common trade-offs of state-of-the-art methods for multi-shape representation (a single model "packing" multiple objects) involve trading modeling accuracy against memory and storage. We show how to encode multiple shapes represented as continuous neural fields with a higher degree of precision than previously possible and with low memory usage. Key to our approach is a recursive hierarchical formulation that exploits object self-similarity, leading to a highly compressed and efficient shape latent space. Thanks to the recursive formulation, our method supports spatial and global-to-local latent feature fusion without needing to initialize and maintain auxiliary data structures, while still allowing for continuous field queries to enable applications such as raytracing. In experiments on a set of diverse datasets, we provide compelling qualitative results and demonstrate state-of-the-art multi-scene reconstruction and compression results with a single network per dataset.

==> tables/fusion.tex <==
\setlength{\tabcolsep}{20pt}
\begin{table}[b]
    \caption{The multiscale feature fusion scheme vs reconstruction quality on HB dataset. At the cost of storage, concatenating features before decoding increases reconstruction accuracy.}
\resizebox{\columnwidth}{!}{%
  \centering
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}[4]{*}{\textbf{Fusion}} & \multicolumn{2}{c}{\textit{Reconstruction}} & \textit{Runtime} & \textit{Size} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-4}  \cmidrule(lr){5-5}        & CD$\downarrow$ & 3D PSNR$\uparrow$ & s$\downarrow$ & MB$\downarrow$ \\
    \midrule
    \textit{Sum}   & 0.046 & 33.61 & 0.11 & 3.2 \\
    \textit{Concatenate} & 0.046 & 34.89 & 0.12 & 3.8 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:fusion}%
\end{table}%

